Salience-Based Adaptive Masking: Revisiting Token Dynamics for Enhanced Pre-training

In this paper, we introduce Saliency-Based Adaptive Masking (SBAM), a novel and cost-effective approach that significantly enhances the pre-training performance of Masked Image Modeling (MIM) approaches by prioritizing token salience. Our method provides robustness against variations in masking ratios, effectively mitigating the performance instability issues common in existing methods. This relaxes the sensitivity of MIM-based pre-training to masking ratios, which in turn allows us to propose an adaptive strategy for `tailored' masking ratios for each data sample, which no existing method can provide. Toward this goal, we propose an Adaptive Masking Ratio (AMR) strategy that dynamically adjusts the proportion of masking for the unique content of each image based on token salience. We show that our method significantly improves over the state-of-the-art in mask-based pre-training on the ImageNet-1K dataset.

==> sec/1_intro_OLD.tex <==
\section{Introduction}
\label{sec:intro}


% \KY{Please see preamble.tex for how we typically collaborate over overleaf. You use the lowercase commands to color your edits so that others can see, and you use the uppercase commands for comments. Also remove colored edits as you go through and find okay}

In recent years, the landscape of self-supervised learning (SSL) has undergone a profound transformation, propelled by the integration of transformer architectures, a methodology first pioneered within the realm of natural language processing. This paradigm shift has not only revolutionized the field but has also paved the way for its application in computer vision, notably through the introduction of the Vision Transformer (ViT). Meanwhile, the inherent data-hungry nature of transformers has led to a growing consensus on the necessity of pre-training these models on pretext tasks, derived purely from the abundance of unlabelled data. A key strategy in this context is the application of masked token modeling, akin to Masked Language Modeling (MLM) employed in NLP. This strategy, adopted as Masked Image Modeling (MIM) for visual data, involves masking a subset of input tokens and training the model to predict these corrupted segments, thereby facilitating a deep contextual comprehension of the unlabelled data.

While Masked Image Modeling (MIM) has significantly advanced self-supervised learning in vision, its conventional approach to randomly selecting tokens for masking falls short of harnessing the full potential of visual data. Unlike in text, where randomness might obscure key semantic units, the visual domain's complexity and token redundancy demand a more strategic masking protocol to ensure model comprehension. This necessity prompts us to explore a refined masking methodology, targeting a deliberate selection process that achieves the goal of image understanding for pre-trained models, thereby bridging the gap in modality-specific pre-training strategies.
%Our endeavor seeks to meticulously evaluate and innovate upon the token masking process, ensuring that each decision to mask is as informed and impactful as possible.


Contemporary masking strategies often grapple with high complexity, burdened by intricate distillation frameworks and auxiliary detection processes. In response to the challenge, this paper introduces a simple yet novel approach that scrutinizes token dynamics, termed \textbf{S}alience-\textbf{B}ased \textbf{A}daptive \textbf{M}asking (\textbf{SBAM}), which aims to strategically select masking locations by discerning perceptual prominence within the visual data. To be specific, the proposed method leverages the directional emphasis from attention mechanisms to identify the image tokens pivotal to the visual context. 
Significantly, our methodology stands apart from conventional attention-based approaches by leveraging the token's outgoing weight to calculate its `token salience' within the image, guiding the prioritization of token masking with precision.
%By employing column-wise scores from the affinity map generated through row-wise softmax operations, this method identifies tokens that significantly contribute to the overall image context, akin to minimizing the reconstruction cost in a non-linear principal component analysis framework.


\input{figs/teaser/item}

Crucially, the brilliance of the SBAM approach lies in its robustness to the varying masking ratios—a notable vulnerability in established baselines like the MAE, which struggles from performance instability with even minor variations in optimized masking ratio. This robustness is attributable to the proposed analytical precision in token dynamics, selectively masking tokens pivotal to the image's entirety. Consequently, SBAM exhibits a diminished likelihood of masking redundant or non-essential segments, offering a refined alternative to the random masking or preceding masking approaches.
%analysis section에 더 풀어서쓰기 - random은 masking ratio가 작아질수록 crucial한 token이 포함될 가능성이 더 적어지지만~
%By concentrating on the significance of tokens, as gauged by their outgoing weights, this approach presents a robust and flexible alternative to conventional methods, adeptly navigating the challenges posed by masking ratio variability.
%This robustness facilitates a paradigm shift in MIM's approach to self-supervised learning, significantly enhancing its adaptability and performance across varying conditions.

Establishing robustness against variations in masking ratios has empowered us to expand the discourse on image masking into a pioneering aspect, introducing an innovative paradigm: an \textbf{A}daptive \textbf{M}asking \textbf{R}atio (\textbf{AMR}). This leap forward acknowledges the inherently diverse visual narratives presented by individual images and adjusts the masking ratio to the varying objects and class sizes. The proposed token salience, reapplied in this context, serves to finely determine the dynamic masking ratio by quantifying the proportion of tokens exhibiting high salience, each tailored to the distinctive image. The proposed AMR implements an adaptive strategy that respects the distinctive complexities of visual data and thus achieves performance gains when applied to various baselines.
%significant performance improvements, marking a significant step forward in the field of self-supervised learning.

In sum, this paper offers a pioneering masking strategy that enhances the robustness and transferability of pre-trained models and sets the stage for a paradigmatic shift in self-supervised learning methodologies. More importantly, the proposed SBAM and AMR approaches can be universally applied across any masked auto-encoder frameworks that rely on token masking, thereby enhancing the efficacy and dynamism of pre-training stages.%성능 얘기 이부분에 넣어야함
%Our contributions, through the introduction of a simplified yet profoundly effective masking strategy, not only bolster the resilience and adaptability of models like MIM and MAE but also pave the way for a transformative shift in self-supervised learning paradigms, with the potential to redefine the landscape of the field. and setting a new standard for adaptability and performance efficiency.

The contributions of this work are threefold:\\
\begin{enumerate}
  \item We present a novel Salience-Based Adaptive Masking method, low in complexity yet rich in discernment, informed by the token salience.
  \item Our approach exhibits unparalleled robustness to masking ratio variations, thereby overcoming the limitations inherent in concurrent baselines.
  \item We introduce the Adaptive Masking Ratio, a pioneering strategy that dynamically adjusts the masking ratio in response to the visual data.
\end{enumerate}
